Teaching-Assistant-in-the-Loop: Improving Knowledge Distillation from Imperfect Teacher Models in Low-Budget Scenarios

There is increasing interest in distilling task-specific knowledge from large language models (LLM) to smaller student models. Nonetheless, LLM distillation presents a dual challenge: 1) there is a high cost associated with querying the teacher LLM, such as GPT-4, for gathering an ample number of demonstrations; 2) the teacher LLM might provide imperfect outputs with a negative impact on the student's learning process. To enhance sample efficiency within resource-constrained, imperfect teacher scenarios, we propose a three-component framework leveraging three signal types. The first signal is the student's self-consistency (consistency of student multiple outputs), which is a proxy of the student's confidence. Specifically, we introduce a ``teaching assistant'' (TA) model to assess the uncertainty of both the student's and the teacher's outputs via confidence scoring, which serves as another two signals for student training. Furthermore, we propose a two-stage training schema to first warm up the student with a small proportion of data to better utilize student's signal. Experiments have shown the superiority of our proposed framework for four complex reasoning tasks. On average, our proposed two-stage framework brings a relative improvement of up to 20.79% compared to fine-tuning without any signals across datasets.

==> previous_method.tex <==
% \section{Methodology}
% Figure \ref{fig:overview} shows the overview of our framework. 
% Our pre-trained student model $M_s$ will first do the few-shot ICL inference on a large unlabeled dataset $U$ and then calculate the student internal signal $s_i$ from the student-generated answer set or the external signal $s_t$ from the judgement of the TA model $M_t$. With the student signals, we distinguish whether this sample is worth annotating by the pre-defined criteria for each type of student signal. If the signal of a sample meets the criteria, we will add it to the annotation bucket $B_a$. After active selection, we ask the teacher model $M_e$ to again use the few-shot ICL to annotate the examples in the annotation bucket. Then the TA model $M_t$ labels the confidence level of the teacher-generated answers. If TA model is confident with the teacher's answer of a question, we will add this question and teacher annotations to the fine-tuning bucket $B_f$. Finally, we fine-tune our student model on the fine-tuning bucket and finish the knowledge distillation. 
% The algorithms outlining this procedure are also presented in Algorithm ~\ref{alg:ta} in Appendix.

% \subsection{Student Signal}

% In the first step, we propose two types of student signals: student internal signal or external signal to judge whether a question is worth to utilize the teacher model to annotate. We will continuously add the questions satisfying the specified criteria to the annotation bucket $B_a$ until the data size in $B_a$ reaches the predefined budget.

% \subsubsection{Student internal signal}
% Motivated by self-consistency work \cite{wang2022self}, we utilize the disagreement number (self-consistency number) as the measurement of the uncertainty of student models. On a given sample $x$ from the unlabeled dataset $U$, instead of greedy decoding approaches, we use stochastic temperature sampling with a large fixed temperature value 0.7 to repeat generations $n$ times and obtain distinct deduction trajectories along with a generated answer set $\{t_{s_0}, t_{s_1}, ..., t_{s_n}\}$ from the student model $M_s$. This process can be formulated as 
% \begin{equation*}
%     t_{s_{0}} \dots t_{s_{n}}=M_{s}(P_{i}\vert\vert x) \dots M_{s}(P_{i}\vert\vert x)
% \end{equation*}
% where $P_i$ is the in-context learning prompt for generating the answer of question $x$.
% We calculate the number of unique answers in the answer set as the disagreement of this training sample and obtain the student internal signal $s_i$. 
% \begin{equation*}
%     s_{i}=\text{Unique Number}(t_{s_{0}} \dots t_{s_{n}})
% \end{equation*}
% For our following experiments, we choose the hyperparameter $n=5$. In Table \ref{table:disagreement_examples} in the Appendix, we present two examples with different numbers of student disagreement.

% \subsubsection{Student external signal}
% \label{sec:student_external}
% Besides the internal signal from the student model, we can also utilize LLM to estimate the uncertainty of the student model, which can be obtained by querying the student model itself for confidence in its own generated answers. However, from observations in previous work, the confidence estimated by LLM itself is prone to be overconfident \cite{diao2023active, si2022prompting}. To solve this drawback, we introduce another LLM, namely the teaching assistant (TA) model $M_t$, which is larger and has more capabilities in complex tasks. After obtaining the answer $t_{s_0}$ from the student model, we provide the TA model with the answer, as well as a crafted confidence prompt $P_c$ containing four confident choices: (a) very confident, (b) confident, (c) not confident, and (d) wrong answer. Then we combine the ``confidence prompt" $P_c$ and the student's output $t_{s_0}$ and feed the concatenation to the TA model $M_t$ to generate the confidence choice $s_{t} = M_{t}(P_{c} \vert\vert t_{s_{0}})$. \textbf{TA-confidence} choice $s_t$ is a categorical variable from the confidence set \{very confident, confident, not confident, wrong answer\}. Details and examples of the confidence prompt $P_c$ and $t_{s_0}$ can be found in Table \ref{table:ta_conf_prompt} and \ref{table:examples_ta_conf} in Appendix.

% \subsubsection{Annotation Criteria}
% \label{sec:annotation}
% When using the student internal signal to actively select samples for annotation, we put the samples with disagreement number $s_i$ equal to 2 or 3 ($\max(s_i) = 5$) in the annotation bucket $B_a$. The intuition of not selecting the most uncertain questions ($s_i$ = 4 or 5) is that even after fine-tuning, the student model cannot correctly complete the hardest questions for challenging tasks. For example, from the previous work, the final fine-tuning accuracy of a 6.7B student model on most reasoning tasks cannot exceed 70\% accuracy \cite{ho2022large}. Therefore, our strategy is to choose the uncertain samples, but not the hardest, in the annotation bucket $B_a$. 

% Similarly, when using the student external signal, we choose questions with TA-confidence $s_t$ equal to ``confident'' or ``not confident'' in the annotation bucket $B_a$. We will stop actively selecting after the number of questions in the annotation bucket reaches the predefined budget.

% We also consider using both two signals at the same time to select the questions for annotation, but the number of questions satisfying both criterion of two signals is small, e.g. only about 1/8 of the whole dataset for the HotpotQA task \cite{yang2018hotpotqa}, causing low sampling efficiency. Therefore, in extensive experiments, we will show two framework variants with either of the student signals and show the effectiveness of the student signals.

% \subsection{Teacher Signal}
% With the desired annotation bucket, we utilize the teacher model $M_e$ to annotate the question $x$ in the annotation bucket $B_a$ with the few-shot ICL. To verify the correctness of teacher annotation $t_e$, we apply the similar TA-confidence as discussed in Section \ref{sec:student_external}. The process of adding TA-confidence can be formulated as
% \begin{equation*}
%     t_e = M_{e}(P_{i}\vert\vert x), \quad s_{e} = M_{t}(P_{c} \vert\vert t_{e})
% \end{equation*}
% where $s_e$ is the TA-confidence of teacher annotations and serve as the teacher signal.
% In the previous work of LLM answer refinement \cite{madaan2023self, shinn2023reflexion}, they use the LLM itself to evaluate the self-generated answers. However, due to the limited budget of calls to the teacher model in our setup, we choose to apply the low-cost TA model to refine the annotations; otherwise, the teacher self-evaluation will cost a large proportion of budgets. We present two examples with questions, teacher annotations as well as TA-confidence in Table \ref{table:confidence_examples} in the Appendix. Unlike the selection criteria for student inference, we choose questions and annotations with TA-confidence equal to ``very confident'' or ``confident'' into the fine-tuning buckets $B_f$ and high confidence from the TA model will reduce noise in the fine-tuning bucket. 


% \subsection{Fine-tune the Student Model}
% After completing the TA verification, we fine-tune the student model with questions and teacher-generated annotations from the fine-tuning bucket. We apply the autoregressive language modeling as well as the cross entropy loss, which is the same as the pretraining objective to fine-tune the student model \cite{gpt-j}.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/two_stage_training.png}
%    \caption{\label{fig:two_stage} \textbf{Overview of two-stage training extension.} We first use 10\% budget to fine-tune the student model and then use the other 90\% to further training the student. We implement both stages with our proposed framework.}
% \end{figure}

% \subsection{Extension: Two-stage Training}
% \label{sec:extension}
% To better utilize the internal signals from the student model, we propose the two-stage training extension to first utilize a small proportion of the training budget to warm up the student and then continue fine-tuning with the remaining budget in the second stage. The motivation behind this extension is that the student model's few-shot ICL can only obtain low accuracy for some tasks, so the uncertainty measurement from the student signal is not reliable. For example, as presented in Section \ref{sec:results}, for HotpotQA task \cite{yang2018hotpotqa}, the accuracy of the student's inference (GPT-J-6B) is only 5.2\%. With such a low accuracy, it is questionable whether student signals can effectively characterize the uncertainty of the student model. Moreover, even if the student signals are reliable, the samples extracted by the student signals are uncertain for the students before fine-tuning, but may not be challenging enough for the student models fine-tuned halfway. 

% To address these challenges, as shown in Figure \ref{fig:two_stage}, we develop a two-stage training. The first stage is the warm-up training, and we use 10\% of the budget to fine-tune the student model with our framework (student signals + teacher signals). For the second stage, we use 90\% of the budget to continue fine-tuning the student model with our framework. We expect that the student signals collected in the second stage are more reliable than the first stage, and more challenging questions collected in the second stage should lead to a more performance boost.

==> prompts/aqua_problems <==
{
    "prompt": [
        {
            "question": "Question: John found that the average of 15 numbers is 40. If 10 is added to each number then the mean of the numbers is? Answer Choices: (a) 50 (b) 45 (c) 65 (d) 78 (e) 64\nA:",
            "rationale": "Let's think step by step. If 10 is added to each number, then the mean of the numbers also increases by 10. So the new mean would be 50.",
            "pred_ans": "A"
        },
        {
            "question": "Question: If a / b = 3/4 and 8a + 5b = 22,then find the value of a. Answer Choices: (a) 1/2 (b) 3/2 (c) 5/2 (d) 4/2 (e) 7/2\nA:",
            "rationale": "Let's think step by step. If a / b = 3/4, then b = 4a / 3. So 8a + 5(4a / 3) = 22. This simplifies to 8a + 20a / 3 = 22, which means 44a / 3 = 22. So a is equal to 3/2.",
            "pred_ans": "B"
        },
        {
            "question": "Question: A person is traveling at 20 km/hr and reached his destiny in 2.5 hr then find the distance? Answer Choices: (a) 53 km (b) 55 km (c) 52 km (d) 60 km (e) 50 km\nA:",
            "rationale": "Let's think step by step. The distance that the person traveled would have been 20 km/hr * 2.5 hrs = 50 km.",
            "pred_ans": "E"
        },
        {
            "question": "Question: How many keystrokes are needed to type the numbers from 1 to 500? Answer Choices: (a) 1156 (b) 1392 (c) 1480 (d) 1562 (e) 1788\nA:",
            "rationale": "Let's think step by step. There are 9 one-digit numbers from 1 to 9. There are 90 two-digit numbers from 10 to 99. There are 401 three-digit numbers from 100 to 500. 9 + 90(2) + 401(3) = 1392.",
            "pred_ans": "B"
        }
    ]
}

==> prompts/csqa_problems <==
{
    "prompt": [
        {
            "question": "Question: What do people use to absorb extra ink from a fountain pen? Answer Choices: (A) shirt pocket (B) calligrapher’s hand (C) inkwell (D) desk drawer (E) blotter\nA:",
            "rationale": "Let's think step by step. The answer must be an item that can absorb ink. Of the above choices, only blotters are used to absorb ink.",
            "pred_ans": "E"
        },
        {
            "question": "Question: What home entertainment equipment requires cable? Answer Choices: (A) radio shack (B) substation (C) television (D) cabinet\nA:",
            "rationale": "Let's think step by step. The answer must require cable. Of the above choices, only television requires cable.",
            "pred_ans": "C"
        },
        {
            "question": "Question: Sammy wanted to go to where the people were. Where might he go? Answer Choices: (A) populated areas (B) race track (C) desert (D) apartment (E) roadblock\nA:",
            "rationale": "Let's think step by step. : The answer must be a place with a lot of people. Of the above choices, only populated areas have a lot of people.",
            "pred_ans": "A"
        },
        {
            "question": "Question: What home entertainment equipment requires cable? Answer Choices: (A) radio shack (B) substation (C) television (D) cabinet\nA:",
            "rationale": "Let's think step by step. The answer should be the place where grocery items are placed before checking out. Of the above choices, grocery cart makes the most sense for holding grocery items.",
            "pred_ans": "B"
        },
        {
            "question": "Question: Google Maps and other highway and street GPS services have replaced what? Answer Choices: (A) united states (B) mexico (C) countryside (D) atlas\nA:",
            "rationale": "Let's think step by step. The answer must be something that used to do what Google Maps and GPS services do, which is to give directions. Of the above choices, only atlases are used to give directions.",
            "pred_ans": "D"
        },
        {
            "question": "Question: Before getting a divorce, what did the wife feel who was doing all the work? Answer Choices: (A) harder (B) anguish (C) bitterness (D) tears (E) sadness\nA:",
            "rationale": "Let's think step by step. The answer should be the feeling of someone getting divorced who was doing all the work. Of the above choices, the closest feeling is bitterness.",
            "pred_ans": "C"
        }
    ]
}

==> prompts/math_word_problems <==
{
    "prompt": [
        {
            "question": "Q: There are 15 trees in the grove. Grove workers will plant trees in the grove today. After they are done, there will be 21 trees. How many trees did the grove workers plant today?\nA:",
            "rationale": "Let's think step by step. There are 15 trees originally. Then there were 21 trees after some more were planted. So there must have been 21 - 15 = 6.",
            "pred_ans": "6"
        },
        {
            "question": "Q: If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot?\nA:",
            "rationale": "Let's think step by step. There are originally 3 cars. 2 more cars arrive. 3 + 2 = 5.",
            "pred_ans": "5"
        },
        {
            "question": "Q: Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total?\nA:",
            "rationale": "Let's think step by step. Originally, Leah had 32 chocolates. Her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39.",
            "pred_ans": "39"
        },
        {
            "question": "Q: Jason had 20 lollipops. He gave Denny some lollipops. Now Jason has 12 lollipops. How many lollipops did Jason give to Denny?\nA:",
            "rationale": "Let's think step by step. Jason started with 20 lollipops. Then he had 12 after giving some to Denny. So he gave Denny 20 - 12 = 8.",
            "pred_ans": "8"
        },
        {
            "question": "Q: Shawn has five toys. For Christmas, he got two toys each from his mom and dad. How many toys does he have now?\nA:",
            "rationale": "Let's think step by step. Shawn started with 5 toys. If he got 2 toys each from his mom and dad, then that is 4 more toys. 5 + 4 = 9.",
            "pred_ans": "9"
        },
        {
            "question": "Q: There were nine computers in the server room. Five more computers were installed each day, from monday to thursday. How many computers are now in the server room?\nA:",
            "rationale": "Let's think step by step. There were originally 9 computers. For each of 4 days, 5 more computers were added. So 5 * 4 = 20 computers were added. 9 + 20 is 29.",
            "pred_ans": "29"
        },
        {
            "question": "Q: Michael had 58 golf balls. On tuesday, he lost 23 golf balls. On wednesday, he lost 2 more. How many golf balls did he have at the end of wednesday?\nA:",
            "rationale": "Let's think step by step. Michael started with 58 golf balls. After losing 23 on tuesday, he had 58 - 23 = 35. After losing 2 more, he had 35 - 2 = 33 golf balls.",
            "pred_ans": "33"
        },
        {
            "question": "Q: Olivia has $23. She bought five bagels for $3 each. How much money does she have left?\nA:",
            "rationale": "Let's think step by step. Olivia had 23 dollars. 5 bagels for 3 dollars each will be 5 x 3 = 15 dollars. So she has 23 - 15 dollars left. 23 - 15 is 8.",
            "pred_ans": "8"
        }
    ]
}
